SoK: Understanding the Attack Surface in Device Driver Isolation Frameworks

Device driver isolation is a promising approach for protecting the kernel from faulty or malicious drivers, but the actual security provided by such frameworks is often not well understood. Recent research has identified Compartment Interface Vulnerabilities (CIVs) in userspace compartmentalized applications, yet their impact on driver isolation frameworks remains poorly understood. This paper provides a comprehensive survey of the design and security guarantees of existing driver isolation frameworks and systemizes existing CIV classifications, evaluating them under driver isolation. The analysis shows that different classes of CIVs are prevalent across the studied drivers under a baseline threat model, with large drivers having more than 100 instances of different CIVs and an average of 33 instances across the studied drivers. Enforcing extra security properties, such as CFI, can reduce the number of CIVs to around 28 instances on average. This study provides insights for understanding existing driver isolation security and the prevalence of CIVs in the driver isolation context, and extracts useful insights that can provide security guidance for future driver isolation systems.

==> Makefile <==
PLOTBITS 	:= $(wildcard plots/*.gnu)

GNUPLOT		:= gnuplot
PS2PDF		:= ps2pdf14

PS2PDFFLAGS_EPS	:= -dEPSCrop -dPDFSETTINGS=/printer \
		   -dColorConversionStrategy=/RGB \
		   -dProcessColorModel=/DeviceRGB \
		   -dEmbedAllFonts=true -dSubsetFonts=true -dMaxSubsetPct=100


FIGEPS		:= $(PLOTBITS:.gnu=.eps)
FIGPDF		:= $(PLOTBITS:.gnu=.pdf)

all: $(FIGEPS) $(FIGPDF)
	pdflatex -shell-escape paper.tex

%.eps: %.gnu
	$(GNUPLOT) \
	$<

# This method produces small PDFs that have tight bounding boxes.
$(PLOTBITS:.gnu=.pdf): %.pdf: %.eps
	$(PS2PDF) $(PS2PDFFLAGS_EPS) $< $@

clean:
	@rm -f paper.pdf
	@rm -f paper.aux paper.bbl paper.log paper.fls paper.dvi paper.blg


==> tex/case-studies.tex <==
\subsection{Case Studies} \label{subsec:case_study}
We select 11 representative drivers spanning the 7 studied driver classes for an in-depth case study of \vulName{}. The case study has two objectives: (1) evaluate the effectiveness of our static analyses and (2) conduct detailed inspections of drivers with or lacking certain \vulName{} types to understand the driver characteristics that contribute to or prevent vulnerabilities. 

\iffalse
\paragraph{\vulName{} auditing effort evaluation} \label{subsec:\vulName{}_auditing_effort}
During the validation process of the \vulName{} discovered by the analyses, we have found that all the taint traces discovered by our taint analysis are valid paths, while not considering the path conditions along the path. After applying the pruning strategy, we are left with the path with highest controllability by the attacker. So, the first step of the auditing is starting from these highly controlled path. 
Second, our generated log files provide the source locations for the taint source, taint sink, and the call path in the kernel that can reach the taint sink, as shown in Listing \ref{lst:example_json_log}.

\begin{listing}[ht]
\fontsize{8}{8}\selectfont
\begin{minted}[xleftmargin=20px, breaklines, linenos]{json}
{
    "id": "173",
    "risky": "arr-idx",
    "acc_path": "i",
    "src": "",
    "dst": "",
    "drv caller": "[ ixgbe_add_rx_frag ], ",
    "call path": " [ixgbe_add_rx_frag->skb_add_rx_frag->
                    skb_fill_page_desc->__skb_fill_page_desc] ",
    "cond_num": "0",
    "isControl": "1",
}
\end{minted}
\caption{Example taint trace log.}
\label{lst:example_json_log}
\end{listing}

In general, it takes around 1 - 2 minutes to fully verify a taint trace with no path condition. For taint traces with multiple path conditions, the required analysis time varies. The longest path that is controllable by the attacker after pruning is xx, which takes about 10 minutes to verify by a graduate student. 
\fi


\paragraph{Evaluate the effectiveness of static analyses} 
\label{subsec:\vulName{}_static_analysis_effectiveness}
To validate how effective our analyses are, we conducted a manual analysis of the cases found.
%
For the \vulName{} instances that are revealed by taint analysis, we only validate the ones that are left after applying the pruning strategy.
%
The reason is that validating all the paths manually is impractical considering the large number of taint traces produced and the complexity of the path conditions, e.g., over 300 more traces for the Ixgbe driver alone, with 74 maximum path conditions for a single trace.
%
%While such a strategy is not complete for checking all the true cases, it is the best effort we can make to assess the effectiveness given the lack of ground truth. 
Tables~\ref{tab:case_study_data_corruption_result} and \ref{tab:case_study_aiv_tv_classification_result} (Appendix~\ref{sec:appendix}) show the overall \vulName{} classification results on the representative drivers. First, we focus on the \vulName{} classes that are revealed by the taint analysis. For each class, we show three numbers: (1) the raw taint traces (NP), (2) the traces remaining after applying our pruning strategy described in Section~\ref{subsec:prune_taint_traces} (P), and (3) traces that are true cases after manual verification (M). A true case is verified in two steps: First, we verify if the source data can actually flow to the sink without being checked. Second, we verify if the trace allows a concrete exploit with a specific source value. The precision of the analysis is computed by dividing M from P. And this shows that the percentage of true cases is 80\%, which indicates that our pruning strategy yields pretty accurate results in revealing taint paths.

\paragraph{Driver design patterns leads/prevents \vulName{}} We observed two key factors contributing to a high number of vulnerability instances in drivers with the following characteristics. First, drivers with larger, more complex interfaces and greater interaction with other kernel components tend to exhibit more instances. Second, drivers that share a substantial amount of state have an increased potential for vulnerabilities around synchronization and data integrity. The network \lstinline{ixgbe} driver and \lstinline{msr} drivers are a good  samples. For ixgbe, it has 83 shared struct types containing 222 shared fields with the kernel, while \lstinline{msr} only has 7 shared struct types containing 7 shared fields. In addition, ixgbe invokes 154 kernel interface functions. MSR, on the contrary, only invokes 18 kernel interface functions. 

\paragraph{Interpret hot data/fields} As mentioned in previous observations, a small percentage of data/fields actually contribute to a large number of \vulName{} instances. We would like to understand why this is the case and the characteristics of such fields. We choose the ixgbe driver as an example. In the ixgbe driver, a boundary pointer parameter \textbf{offset} contributes to four risky vectors (ptr-deref, pointer-offset/arr-index, integer over/underflow, sensitive-kernel-api). The code accessing this data is shown in Listing~\ref{lst:example_of_multi_risky_classes_data}. Lines 6 and 8 are pointer dereference cases, and Line 16 has a potential integer overflow, as the condition depends on data derived from the offset. At Line 25, a memory copy API also uses a pointer \textbf{p\_off}, which is computed from the offset. By manipulating the offset pointer and its dereferenced value, an attacker can affect all these risky sinks. To prevent the \vulName{} associated with this data, we need to make sure the proper checks are performed when the data is passed to the kernel initially. However, the pointer dereference itself is not checked first to make sure the pointer is not NULL, and there are no checks to ensure the value pointed by the offset is within the expected range. The \textbf{offset} parameter grants the attacker with multiple ways to attack the kernel.


\begin{listing}[h]
\scriptsize
\begin{minted}[xleftmargin=20pt,linenos,escapeinside=||]{c}
int ipv6_find_hdr(const struct sk_buff *skb,
        unsigned int *offset, ...) {
  unsigned int start = skb_network_offset(skb)
        + sizeof(struct ipv6hdr);
  ...
  // pointer dereference
  if (*offset) {
    start = *offset + sizeof(struct ipv6hdr);
  }
  ...
  hp = skb_header_pointer(..., start, ...);
}

void* skb_header_pointer(..., int offset, ...) {
  // offset is used to compute a condition
  if (hlen - offset >= len)
    return data + offset;
  if (skb_copy_bits(skb, offset, buffer, len) < 0)
  ...      
}

int skb_copy_bits(const struct sk_buff *skb,
        int offset, void *to, int len) {
  ... 
  // p_off  is derived from offset
  memcpy(to + copied, vaddr + p_off, p_len);
}


\end{minted}
\caption{Example of multi-risky class data.}
\label{lst:example_of_multi_risky_classes_data}
\end{listing}


\iffalse
\section{Evaluating Driver Isolation Frameworks Against \vulName{}}
\label{sec:defense_strategy_for_\vulName{}}
In this section, we discuss whether existing driver isolation frameworks can 
effectively prevent the \vulName{}.
%
Current driver isolation frameworks provide strong policy enforcement mechanisms. However, manual work is needed to determine where the policy needs to be enforced.
%
Even with strong policy enforcement, data-only attacks are still possible because the data passed across the boundary is not always correctly validated.

\paragraph{Corrupted pointer value} Attacker attempts to synchronize corrupted pointer value to the kernel with this \vulName{}.
%
Such attacks are preventable in frameworks such as Microdrivers~\cite{microdrivers} and KSplit~\cite{ksplit}, as they maintain private shadow copies of data structures to enforce isolation and only synchronize the shared states.
%
%For pointer type, such framework will have alternative pointer repsentation
%in different compartment. Thus, when a malicious driver corrupts a pointer value, %it corrupts the representation at its end. When it passes this value to wrapper %function, such corrupted pointer is likely to be rejected because the framework %will fail the pointer lookup after domain crossing.

Frameworks such as HAKC~\cite{hakc} use pointer authentication~\cite{pac-it-up} to 
prevent a pointer from being corrupted directly by unauthorized compartments.
%
However, if the kernel trusts a driver and expects it to modify a pointer, the corrupted driver can still bypass the policy enforcement in HAKC.
%
LXFI~\cite{lxfi} faces similar issues. Even though LXFI enforces write capability, it only prevents the corrupted driver from directly modifying the pointer address.
%
However, an attacker can still corrupt the data pointed to by the pointer.

%as it uses capabilities to enforce accesses on shared pointers. However, it's not 
%sufficient to prevent the attacker from corrupting the pointer value

\paragraph{Corrupted pointer offset or buffer index}
Pointer offsets and buffer indices have  implicit invariants on the bounds: 
the value should never exceed the bounds of the buffer.
%
Data structures, such as \lstinline{sk_buff}, have invariants that involve more variables~(e.g., \lstinline{skb->tail} field should be always within the \lstinline{skb->head + skb->len}.
%
Extracting such invariants automatically is a complex problem, but it can be 
partially addressed with invariant inference techniques, such as 
Daikon~\cite{daikon}
as shown by Butt et al.~\cite{protecting_comm_kernel_from_vulnerable_driver}.
%
Additionally, inferring missing checks with voting methods \cite{Lu_missing_check_constraints_inference} is also a potential solution.
%This can be leverage to learn the correct checks from all checks on a data across the whole problem, and then 
%detect missing checks upon the use of the data.

%\paragraph{Data structure invariants}
%Different driver class should obey a set of invariants on the shared data. 

\paragraph{Data used in sensitive APIs}
The kernel, through a set of sensitive APIs, provides complex functionalities to the other subsystems~(paragraph ~\ref{para:sensitive-apis}).
%
The concrete consequence of misusing them differs depending
on the class and nature of the corresponding API.
%
For memory APIs, corrupting the pointers used in the API grants arbitrary read/write capabilities, and corrupting the size parameter allows control over the amount of data that can be modified or copied~\cite{CIVScope}.
%
By corrupting arguments to the power management APIs, an attacker can manipulate the device's power.
%
Corrupting interrupt APIs, an attacker can generate spurious interrupts or suppress interrupts to other devices, leading to denial of service attacks.
%
In general, our study suggests that sensitive APIs should never be directly exposed to the drivers.
%
Wrapper functions are needed to perform the necessary
sanity checks on the data passed to the API.
%
This can be achieved easily for isolation frameworks that use shadow copies 
as they already have trampoline functions for marshaling/unmarshaling data~\cite{microdrivers,ksplit}. %Such functions are perfect places to insert necessary
%sanity checks.
\fi

\iffalse
\begin{table*}[h]
 \resizebox{\textwidth}{!}{%
\begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Vulnerability Type (positive/found)} & MSR                   & acpi\_power\_meter      & dm-zero               & null\_blk              & sb\_edac               & sfc                   & usb-f-mass-storage    & skx\_edac              & alx                   & dummy                 & mgag200               \\ \hline
\textbf{Memory Safety}                       & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\hspace{1em} - DC1: mem-ptr-dereference                          & 1                     & 0                     & 0                     & 1/1                   & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 3                     \\ \hline
\hspace{1em} - mem-type-confusion                           & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     \\ \hline
\textbf{Sensitive-API}                       & 1/3                   & 2                     & 0                     & 3/3                   & 0                     & 3                     & 0                     & 0                     & 1                     & 0                     & 4                     \\ \hline
\textbf{Control Data}                        & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\hspace{1em} - loop                                         & 0                     & 0                     & 0                     & 0                     & 3                     & 1                     & 0                     & 5                     & 0                     & 0                     & 1/2                   \\ \hline
\hspace{1em} - risky-branch                                 & 0                     & 3                     & 0                     & 0/3                   & 0/5                   & 1/2                   & 1                     & 0/5                   & 0                     & 0                     & 0/7                   \\ \hline
\textbf{Arith Errors}                        & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\hspace{1em} - div-by-zero                                  & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     \\ \hline
\hspace{1em} - int overflow/underflow                       & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     & 0                     \\ \hline
\textbf{Corrupted concurret primatives}      & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\hspace{1em} - lock under condition                         & 0                     & 0                     & 0                     & 0                     & 0                     & 3                     & 0                     & 0                     & 0                     & 0                     & 0                     \\ \hline
\hspace{1em} - loop in cs                                   & 0                     & 0                     & 0                     & 2                     & 0                     & 3                     & 0                     & 0                     & 0                     & 0                     & 0                     \\ \hline
\textbf{Protocol violation}                  & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\hspace{1em} - kernel interface called under conditional    & 18                    & 43                    & 2                     & 80                    & 144                   & 583                   & 96                    & 97                    & 43                    & 2                     & 163                   \\ \hline
\hspace{1em} - reachable bug on (controlled/total)          & 0/5                   & 2/16                  & 0/5                   & 52/81                 & 0/3                   & 726/1226              & 3/27                  & 0/4                   & 71/91                 & 0/5                   & 3/68                  \\ \hline
\hspace{1em} - life violation via reference count           & 0                     & \multicolumn{1}{l|}{} & 2                     & 2                     & 0                     & 5554                  & 109                   & 0                     & 195                   & 2                     & 27                    \\ \hline
\hspace{1em} - corrupted driver callback return             & 9                     & 10                    & 0                     & 33                    & 0                     & 952                   & 9                     & 0                     & 10                    & 0                     & 150                   \\ \hline
\end{tabular}
}
\end{table*}


\begin{table*}[ht]
    \centering
    % First Subtable
    \begin{subtable}{\textwidth}
        \centering
        \resizebox{0.8\textwidth}{!}{%
        \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|}
            \hline
            & \textbf{ixgbe} & \textbf{alx} & \textbf{null\_net} & \textbf{dm\_zero} & \textbf{msr} & \textbf{xhci\_hcd} & \textbf{nvme} & \textbf{sb\_edac} & \textbf{can\_raw} \\
            \hline
            No. SLOC & 27K & 3K & 194 & 54 & 218 & 10K  &  & 2K & 615 \\
            \hline
            No. Kernel boundary functions & 113 & 52 & 16 & 4 & 15 & 43 & 84 & 13 & 27\\
            \hline
            No. Driver registered callbacks & 92 & 24 & 10 & 2 & 4 & 27 & 24 & 1 & 8\\
            \hline
            No. Boundary parameter & 223 & 76 & 19 & 4 & 35 & 73 & 146 & 28 & 40\\
            \hline
            No. Shared struct & 68 & 29 & 2 & 8 & 6 & 31 & 39 & 11 & 10\\
            \hline
        \end{tabular}
        }
        \caption{Driver overall statistics}
        \label{tab:representative-driver-overall-statistics}
    \end{subtable}
    
    \vspace{1em} % Add vertical space between subtables
    
    % Second Subtable
   \begin{subtable}{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & \multicolumn{2}{c|}{\textbf{ixgbe}} & \multicolumn{2}{c|}{\textbf{alx}} & \multicolumn{2}{c|}{\textbf{null\_net}} & \multicolumn{2}{c|}{\textbf{dm\_zero}} & \multicolumn{2}{c|}{\textbf{msr}} & \multicolumn{2}{c|}{\textbf{xhci\_hcd}} & \multicolumn{2}{c|}{\textbf{nvme}} & \multicolumn{2}{c|}{\textbf{sb\_edac}} & \multicolumn{2}{c|}{\textbf{can\_raw}} \\
        \hline
        \textbf{Boundary parameters} & \multicolumn{2}{c|}{223} & \multicolumn{2}{c|}{76} & \multicolumn{2}{c|}{19} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{35} & \multicolumn{2}{c|}{73} & \multicolumn{2}{c|}{146} &\multicolumn{2}{c|}{28} & \multicolumn{2}{c|}{40}  \\
        \hline
        \hline
        & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune \\
        \hline
        \textbf{Ptr Fields} & & & & & & & & & & & & & & & & & & \\
        \hline
        \hspace{1em} - Ptr Read & 1 & 0/0 & 1 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 1 & 0/0 & 1 & 0/0 & 0 & 0/0 & 0 & 0/0 \\
        \hline
        \hspace{1em} - Ptr Update & 1 & 0/0 & 1 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 1 & 0/1 & 1 & 0/1 & 2 & 0/2 & 0 & 0/0 \\
        \hline
        \textbf{Non-ptr Fields} & & & & & & & & & & & & & & & & & & \\
        \hline
        \hspace{1em} - Array Index & 5 & 0/1 & 2 & 0/0 & 1 & 0/0  & 0  & 0/0 & 4 & 0/0 & 1 & 0/0 & 0 & 0/0 & 2 & 0/0 & 3 & 0/0 \\
        \hline
        \hspace{1em} - Numeric Arith & 8 & 0/2 & 3 & 1/0 & 2 & 0/0 & 0 & 0/0 & 6 & 0/0 & 6 & 0/3 & 7 & 0/2 & 2 & 0/0 & 3 & 0/0 \\
        \hline
        \textbf{Branch} & 4 & 0/2 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 1 & 0/1 & 4 & 2/0 & 2 & 0/2 & 0 & 0/0 \\
        \hline
        \textbf{Risky Kernel Functions} & 10 & 1/4 & 3 & 0/1 & 1 & 0/0 & 0 & 0/0 & 1 & 0/0 & 6 & 0/2 & 2 & 0/2 & 5 & 0/5 & 3 & 0/1 \\
        \hline
    \end{tabular}
    }
    \caption{DIBV classification for boundary parameters}
    \label{tab:representative-driver-boundary-parameter-DIBV-classification}
\end{subtable}

\vspace{1em} % Add vertical space between subtables
   \begin{subtable}{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & \multicolumn{2}{c|}{\textbf{ixgbe}} & \multicolumn{2}{c|}{\textbf{alx}} & \multicolumn{2}{c|}{\textbf{null\_net}} & \multicolumn{2}{c|}{\textbf{dm\_zero}} & \multicolumn{2}{c|}{\textbf{msr}} & \multicolumn{2}{c|}{\textbf{xhci\_hcd}} & \multicolumn{2}{c|}{\textbf{nvme}} & \multicolumn{2}{c|}{\textbf{sb\_edac}} & \multicolumn{2}{c|}{\textbf{can\_raw}} \\
        \hline
        \textbf{KRDU fields} & \multicolumn{2}{c|}{132} & \multicolumn{2}{c|}{61} & \multicolumn{2}{c|}{21} & \multicolumn{2}{c|}{0} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{40} & \multicolumn{2}{c|}{24} &\multicolumn{2}{c|}{10} & \multicolumn{2}{c|}{7}  \\
        \hline
        \hline
        & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune \\
        \hline
        \textbf{Ptr Fields} & & & & & & & & & & & & & & & & & & \\
        \hline
        \hspace{1em} - Ptr Read & 5 & 0/5 & 4 & 2/2 & 3 & 0/2 & 0 & 0/0 & 0 & 0/0 & 1 & 0/0 & 5 & 0/2 & 4 & 0/4 & 3 & 0/2 \\
        \hline
        \hspace{1em} - Ptr Update & 3 & 0/3 & 3 & 0/3 & 2 & 0/2 & 0 & 0/0 & 0 & 0/0 & 1 & 0/1 & 3 & 0/0 & 3 & 2/1 & 3 & 0/2 \\
        \hline
        \textbf{Non-ptr Fields} & & & & & & & & & & & & & & & & & & \\
        \hline
        \hspace{1em} - Array Index & 6 & 0/1 & 1 & 0/0 & 0 & 0/0  & 0 & 0/0 & 0 & 0/0 & 1 & 0/0 & 1 & 0/0 & 0 & 0/0 & 0 & 0/0 \\
        \hline
        \hspace{1em} - Numeric Arith & 15 & 0/12 & 4 & 0/4 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 6 & 0/3 & 2 & 1/0 & 1 & 0/1 & 0 & 0/0 \\
        \hline
        \textbf{Branch} & 14 & 1/8 & 5 & 0/4 & 3 & 0/3 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 5 & 0/1 & 1 & 0/1 & 3 & 0/0 \\
        \hline
        \textbf{Risky Kernel Functions} & 6 & 0/1 & 1 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 3 & 0/0 & 5 & 0/0 & 0 & 0/0 & 3 & 0/0 \\
        \hline
    \end{tabular}
    }
    \caption{DIBV classification for KRDU fields}
    \label{tab:representative-driver-shared-fields-DIBV-classification}
\end{subtable}

\vspace{1em} % Add vertical space between subtables

  % Third Subtable
    \begin{subtable}{\textwidth}
    \centering
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
        \hline
        & \multicolumn{2}{c|}{\textbf{ixgbe}} & \multicolumn{2}{c|}{\textbf{alx}} & \multicolumn{2}{c|}{\textbf{null\_net}} & \multicolumn{2}{c|}{\textbf{dm\_zero}} & \multicolumn{2}{c|}{\textbf{msr}} & \multicolumn{2}{c|}{\textbf{xhci\_hcd}} & \multicolumn{2}{c|}{\textbf{nvme}} & \multicolumn{2}{c|}{\textbf{sb\_edac}} & \multicolumn{2}{c|}{\textbf{can\_raw}} \\
        \hline
        \textbf{No. Kernel Boundary Functions} & \multicolumn{2}{c|}{113} & \multicolumn{2}{c|}{52} & \multicolumn{2}{c|}{16} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{15} & \multicolumn{2}{c|}{43} & \multicolumn{2}{c|}{84} & \multicolumn{2}{c|}{13} & \multicolumn{2}{c|}{27} \\
        \hline
        \textbf{No. Risky Kernel Functions Reached} & 126 & 6/120 & 77 & 3/74 & 37 & 0/37 & 1 & 0/1 & 26 & 0/26 & 18 & 4/14 & 149 & 144/5  & 9 & 1/8 & 18 & 0/18 \\
        \hline
        & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune & No Prune & Prune \\
        \hline
        \hspace{1em} Memory & 27 & 27/0 & 12 & 11/0 & 12 & 7/0 & 1 & 0/0 & 4 & 4/0 & 3 & 3/0 & 27 & 24/0 & 2 & 2/0 & 11 & 8/0 \\
        \hline
        \hspace{1em} Concurrency & 36 & 35/0 & 7 & 7/0 & 13 & 13/0 & 0 & 0/0 & 10 & 9/0 & 0 & 0/0 & 24 & 21/0 & 4 & 4/0 & 6 & 5/0 \\
        \hline
        \hspace{1em} Timer & 10 & 6/0 & 5 & 1/0 & 4 & 0/0 & 0 & 0/0 & 0 & 0/0  & 4 & 1/0 &  34 & 14/0 & 0 & 0/0 & 1 & 0/0 \\
        \hline
        \hspace{1em} DMA & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 \\
        \hline
        \hspace{1em} Refcount & 13 & 5/0 & 5 & 4/0 & 2 & 0/0 & 0 & 0/0 & 9 & 7/0 & 0 & 0/0 & 17 & 9/0 & 0 & 0/0 & 0 & 0/0 \\
        \hline
        \hspace{1em} Bus Management & 33 & 23/0 & 43 & 18/0 & 0 & 0/0 & 0 & 0/0 & 0 & 0/0 & 7 & 1/0 & 36 & 13/0 & 2 & 1/0 & 0 & 0/0\\
        \hline
    \end{tabular}
    }
    \caption{Distribution of kernel boundary functions}
    \label{tab:representative-driver-kernel-boundary-functions-distribution}
\end{subtable}

\caption{Selective driver DIBV classification results}
\label{table:driver-specific-DIBV-result}
\end{table*}
\fi


\iffalse
\begin{table*}[h]
    \centering
    \caption{Analysis of Risky Operations in Device Driver Isolation}
    \label{tab:risky_operations}
    \begin{tabular}{|m{3cm}|m{3cm}|m{2cm}|m{2.5cm}|m{3cm}|m{2.5cm}|}
        \hline
        Risky Operation & Corrupted States Supplied By Driver & Invocation Origin & Protection? & Check Sufficient? & Atomic Check-Operation? \\
        \hline
        \hline
        Operation & Kernel boundary crossing & Kernel driver isolation boundary & Yes & / & No \\
        \hline
    \end{tabular}
\end{table*}
\fi


\iffalse
\subsection{Common DIBV Patterns} \label{sec:common_DIBV_patterns}

As shown in Table \ref{table:driver-specific-DIBV-result}, the risky class with the large number (attacker surface) is corrupting data used in risky kernel functions. The branch and numeric arithmetic types of values are also common. 

By performing an in-depth investigation on the representative drivers, we have summarize the following DIBV patterns. 

\subsubsection{Insecure Data Flow} \label{sec:insecure_data_flow_conclusion}
\paragraph{Unchecked Pointer Dereferences} From the representative drivers, pointer related operations, such as dereferencing a pointer or updating the pointed objects (Ptr read and Ptr write), account for up to 29\% (33/111) of the classified DIBVs. However, when validating such cases, we found that all pointer operations are properly guarded within the kernel context. Before use, the kernel normally performs corresponding checks on the accessed pointer to prevent null pointer dereferences, as shown in listing~\ref{lst:pointer_deref_with_protection}.

\begin{listing}[!ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
// risky field dev->parent is dereferenced
if (dev->parent && device_is_not_partition(dev)) {
  error = sysfs_create_link..., &dev->parent->kobj, "device");
}
\end{minted}
\caption{Pointer dereference with protection.}
\label{lst:pointer_deref_with_protection}
\end{listing}



\paragraph{Unbounded Numeric Field Manipulation}
Unbounded numeric operations could lead to potential integer overflows or underflows. In our classification, 26\% (29/111) of DIBVs arise from risky numeric operations. When examining these operations, the goal is to identify potentially missing checks on the results of unsafe arithmetic.

Our investigation reveals that while most cases seem to enable unguarded use of numeric values produced from unsafe numeric operations, the kernel often employs some validation of the inputs upfront. For instance in Listing~\ref{lst:bounds_check_before_numeric_operations}, the tainted sec and nsec values from a driver are checked to be below \texttt{MAX\_SEC\_IN\_JIFFIES} before use in arithmetic. This ensures the result cannot be manipulated by a malicious driver.

\begin{listing}[!ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
unsigned long __timespec64_to_jiffies(u64 sec, long nsec)
{
	if (sec >= MAX_SEC_IN_JIFFIES){
		sec = MAX_SEC_IN_JIFFIES;
		nsec = 0;
	}
	return ((sec * SEC_CONVERSION) + (((u64)nsec * NSEC_CONVERSION) >> (NSEC_JIFFIE_SC - SEC_JIFFIE_SC))) >> SEC_JIFFIE_SC;
}
\end{minted}
\caption{Bounds range on risky numeric operations.}
\label{lst:bounds_check_before_numeric_operations}
\end{listing}

However, we also identified cases where results of numeric operations are not properly guarded before use. Listing~\ref{lst:missing_bounds_check_before_numeric_operations} shows an example missing range checks in the ixgbe driver.

Here, the parameter i from the driver is directly passed to the kernel function \texttt{skb\_fill\_page\_desc} without validation. This value affects the \texttt{nr\_frags} field in the shared skb info struct, used by various \texttt{sk\_buff} helpers like \texttt{\_\_skb\_pagelen}. In \_\_skb\_pagelen, nr\_frags controls the loop at line 7 without checks, allowing a malicious driver to manipulate the return len value and cause further issues.

\begin{listing}[!ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
void skb_fill_page_desc(struct sk_buff *skb, int i, ...)
{
    ...
    skb_shinfo(skb)->nr_frags = i + 1;
}

unsigned int __skb_pagelen(const struct sk_buff *skb)
{
    ...
    for (i = skb_shinfo(skb)->nr_frags - 1; (int)i >= 0; i--)
        len += skb_frag_size(&skb_shinfo(skb)->frags[i]);
    return len;
}
\end{minted}
\caption{Missing range check on risky numeric operations.}
\label{lst:missing_bounds_check_before_numeric_operations}
\end{listing}

In our study, we have found that 6/29 of risky numeric operations are missing proper checks, which indicates that the compromised driver could potentially utilize such oversight to launch attacks towards the kernel.

\paragraph{Missing checks for data used in risky kernel functions}
The driver invokes kernel boundary functions which transitively call risky kernel APIs to interact with kernel resources. Corrupted data from a malicious driver flowing to such APIs could affect their behavior. For example, kmalloc takes a size parameter that could be manipulated to allocate excessive or insufficient kernel memory. Such data accounts for 15\% (17/111) of DIBVs.

Our examination revealed that in 76\% (13/17) of cases, data flows to kernel APIs without proper input validation. Further analysis showed 10/13 instances were risky kernel functions directly invoked by the driver itself. For example in Listing~\ref{lst:missing_checks_risky_kernel_function}, the xhci-hcd driver directly calls kmalloc where the size is controlled by the driver. Even with checks in the driver, an attacker could likely bypass them. This suggests risky kernel functions should not be directly callable by external drivers. Instead, wrapper functions should be introduced in the kernel to validate arguments before invoking privileged APIs. For instance, a kmalloc wrapper would sanitize the size parameter before allocating kernel memory. Such refactoring limits the attack surface exposed to drivers.

\begin{listing}[!ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
int xhci_setup_msix(struct xhci_hcd *xhci)
{
    ...
    xhci->msix_entries = kmalloc((sizeof(struct msix_entry))*xhci->msix_count, GFP_KERNEL);
    ...
}
\end{minted}
\caption{Missing checks on arguments to risky kernel functions.}
\label{lst:missing_checks_risky_kernel_function}
\end{listing}

\paragraph{Unbounded Array Indexing}
Array indexing accounts for only 1\% (2/111) of classified DIBVs. However, improper indices pose a direct buffer overflow threat. Unfortunately, both discovered instances lack proper index validation by the kernel. Listing~\ref{lst:missing_check_on_array_index} shows  \texttt{\_\_skb\_fill\_page\_desc} directly using the driver parameter i to index the frags array in the skb shared info struct. This enables immediate out-of-bounds access under attacker control. Specifically, a malicious driver could provide arbitrary values for i to trigger an integer overflow in the array index. This could allow overwriting adjacent fields in the skb struct to corrupt integrity. 

\begin{listing}[!ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
// kernel function
void __skb_fill_page_desc(struct sk_buff *skb, int i, ...) 
{
    skb_frag_t *frag = &skb_shinfo(skb)->frags[i];
    ...
}
\end{minted}
\caption{Missing checks on array index.}
\label{lst:missing_check_on_array_index}
\end{listing}


\subsubsection{Insecure Control Flow}

\paragraph{Corrupted Callbacks} When issuing callbacks provided by the driver, the kernel performs a null check on function pointers to prevent crashes. However, as discussed in Section \ref{sec:common_DIBV_patterns}, malicious components could corrupt valid callback pointers to hijack control flow. 

\paragraph{Violating Kernel Driver Protocols} In Table \ref{tab:representative-driver-kernel-boundary-functions-distribution}, we show the classes of risky kernel functions that drivers can transitively invoke via kernel boundary functions. For instance, drivers invoked memory functions, reference counting, bus management functions etc. In many cases, the ordering and preconditions expected by these functions could be violated by a malicious driver.


\para{Invoking single kernel boundary function.}
In isolation API abuse, the attacker can invoke a single kernel boundary function and pass corrupted arguments. If the corrupted data reaches risky kernel operations, various attacks are possible. Listing \ref{lst:API_abuse_example} shows an example in the ixgbe net device driver revealed by our analysis. The driver function \texttt{ixgbe\_ptp\_rx\_pktstamp} calls the kernel helper \texttt{skb\_copy\_bits} and passes a tainted \texttt{offset} value controlled by the attacker.

Inside \texttt{skb\_copy\_bits}, this offset is propagated via \texttt{skb\_copy\_from\_linear\_data\_offset} to the \texttt{memcpy} API on line 15. By controlling the offset, the attacker can manipulate what data is copied to the \texttt{skb} pointer, enabling arbitrary memory read in the kernel. This illustrates how even standard kernel helper functions can be abused by compromise drivers passing malformed arguments. The tainted data flows through multiple levels of indirection before reaching a dangerous sink operation.

\begin{listing}[ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
// driver function
void ixgbe_ptp_rx_pktstamp(struct ixgbe_q_vector *q_vector,
			   struct sk_buff *skb)
{
  ...
  skb_copy_bits(skb, skb->len - IXGBE_TS_HDR_LEN, &regval, IXGBE_TS_HDR_LEN);
  ...
}

// kernel functions
int skb_copy_bits(const struct sk_buff *skb, int offset, void *to, int len)
{
  if ((copy = start - offset) > 0) {
    ...
    skb_copy_from_linear_data_offset(skb, offset, to, copy);
    ...
  }
}

void skb_copy_from_linear_data_offset(const struct sk_buff *skb, const int offset, void *to, const unsigned int len)
{
	memcpy(to, skb->data + offset, len);
}

\end{minted}
\caption{Abuse single kernel boundary API invocation example.}
\label{lst:API_abuse_example}
\end{listing}

\para{Invoking multiple kernel boundary functions.}
With arbitrary execution in the driver domain, the attacker can compound multiple boundary API calls to violate assumptions in kernel logic. This manifests as high-order vulnerabilities where attacker-controlled state from one call influences subsequent calls \cite{high_order_taint_vul_OS}. One specific form we consider is protocol violations - calling kernel functions in orders that break ordering assumptions. For instance, \texttt{kfree} should follow \texttt{kmalloc}, otherwise double-free bugs occur. Detecting such violations is challenging as it requires modeling the ground truth ordering, which is extremely hard to infer in highly concurrent code like the kernel.

Listing \ref{lst:API_abuse_example_2} shows an example found by our analysis. In network drivers, the \texttt{sk\_buff} struct represents packet data used across the kernel networking stack. A compromised driver can trigger premature freeing of a \texttt{sk\_buff}, causing later operations that dereference it to trigger use-after-free bugs. In the example, the driver \texttt{ixgbe\_xmit\_frame} calls \texttt{dev\_kfree\_skb\_any} on Line 4 to free the packet buffer. Later, the kernel \texttt{skb\_clone} function dereferences the freed \texttt{skb} leading to a use-after-free. By modeling kernel API dependencies, we can detect where compromised sequences violate expected state lifetimes.

\begin{listing}[ht]
\fontsize{6}{6}\selectfont
\begin{minted}[xleftmargin= 20px, linenos, breaklines]{c}
// driver function

// kernel functions

\end{minted}
\caption{Abuse multiple kernel boundary API invocation to violate driver kernel communication protocol.}
\label{lst:API_abuse_example_2}
\end{listing}

\begin{listing}[ht]
{\fontsize{6}{11}\selectfont
\begin{minted}[xleftmargin= 22px,linenos, breaklines]{c}
void skb_add_rx_frag(struct sk_buff *skb, ... , unsigned int truesize)
{
	...
	skb->truesize += truesize;
}

static inline struct sk_buff *skb_clone_and_charge_r(struct sk_buff *skb, struct sock *sk)
{
    ...
		if (sk_rmem_schedule(sk, skb, skb->truesize)) {
			...
			return skb;
		}
		__kfree_skb(skb);
	}
	return NULL;
}

static inline bool
sk_rmem_schedule(struct sock *sk, struct sk_buff *skb, int size)
{
	if (!sk_has_account(sk))
		return true;
	return size<= sk->sk_forward_alloc ||
		__sk_mem_schedule(sk, size, SK_MEM_RECV) ||
		skb_pfmemalloc(skb);
}
\end{minted}
\caption{Updates to kernel-private fields through kernel interface functions.}
\label{lst:API_abuse_example}
\end{listing}

For example, \mintinline{c}{skb_add_rx_frag}, a kernel interface function
shown in Listing~\ref{lst:API_abuse_example}, changes the value of
\mintinline{c}{skb->truesize}, a kernel private field. In another portion
of the network subsystem \mintinline{c}{kb_clone_and_charge_r},
\mintinline{c}{skb->truesize} is used in a branching condition. If a driver
calls \mintinline{c}{skb_add_rx_frag}, it can change the value of
\mintinline{c}{skb->truesize} and later influence the control flow to run
risky kernel operations like the free operation shown on line 14.
\gtan{Something seems wrong with the code: the free is outside of the if
  conditional. Also, try to use \ldots as much as possible to make the code
  simpler, e.g., on unrelated parameters and code. }
\mennis{}

\gtan{Don't feel this example adds too much; can remove.}
The \mintinline{c}{kb_add_rx_frag} function demonstrates how a driver
can transitively manipulate non-shared kernel state like
\mintinline{c}{sk_buff} structures, even through error handling
paths. This represents a broader threat---seemingly harmless driver
operations can corrupt critical internal structures in unintended
ways.

\para{Kernel-protocol violation} The second category involves calls to
kernel API functions at unexpected time, unexpected orders, or unexpected times of invocation.
The driver normally requires a rich set of kernel risky functions to accomplish 
its goals, such as memory management (kmalloc/kfree/referce counting), or timer, 
concurrency primitives. 

Listing~\ref{lst:API_abuse_example2}, we show a DIBV which involves repeatedly invoking
\texttt{kobject\_put} and causes potential user-after-free attacks. 
In the driver function \texttt{\_\_ixgbe\_enable\_sriov}, there is a for loop at line 5, within which 
a kernel function called \texttt{pci\_dev\_put} is used to decrease the reference for an \texttt{vfdev}
object. 
Here, suppose the attacker has control on the \texttt{num\_vfs} field, 

One example of a kernel function with this capability is shown in
Listing~\ref{lst:API_abuse_example2}.  \mintinline{c}{free_irq}, a
kernel interface function, frees an interrupt request handler. If a
driver is able to invoke this function, then an interrupt request
handler is freed while the kernel expects it allocated.

We uncovered a subset of these kernel interfance functions with with
memory management capabilities that were direct calls to allocation
and deallocation functions, giving the driver near complete control of
the heap of the kernel.


\subsection{Example of shared state corruption attacks}
Modern isolation frameworks use synchronization hooks to maintain consistent shared state between the kernel and isolated drivers. There are two main types of hooks: First, boundary crossings on interface calls and returns synchronize arguments and return values. This is discussed in the kernel isolation API abuse vector.

Second, concurrently accessed shared data objects have lock release hooks. The kernel holds the master copy of such shared objects. Drivers acquire locks before accessing them. When acquiring/releasing a lock, changes are synchronized to/from the driver's local copy back to the kernel master copy \cite{ksplit, microdrivers}. This ensures that the kernel and driver have a consistent view on the states of these shared objects. 

List~\ref{lst:synchronize_corrupted_shared_states} shows an example where a compromised driver corrupts the shared \texttt{skb->data\_len} field (line 6) and synchronizes this back to the kernel when releasing the lock. By repeatedly triggering this, the attacker can control the values synchronized back.

Later in \texttt{copy\_skb}, the kernel reads this corrupted length value (line 15) and uses it to allocate a new skb copy. This allows the attacker to consume excess kernel memory by forcing larger allocations.

\begin{listing}[ht]
\fontsize{7}{7}\selectfont
\begin{minted}[xleftmargin=21px, breaklines, linenos]{c}
// driver function
void ixgbe_pull_tail(struct ixgbe_ring *rx_ring, struct sk_buff *skb)
{
  unsigned int pull_len;
  ...
  skb->data_len -= pull_len;
  ...
}

// kernel function
struct sk_buff *skb_copy(const struct sk_buff *skb, gfp_t gfp_mask)
{
  ...
  unsigned int size = skb_end_offset(skb) + skb->data_len;
  
  struct sk_buff *n = __alloc_skb(size, gfp_mask, ...);
}

\end{minted}
\caption{Synchronize corrupted shared states.}
\label{lst:synchronize_corrupted_shared_states}
\end{listing}

\subsection{Examples of shared data corruption attack} \label{sec:shared_data_corruption_attack}
\gtan{Move these examples to a later section.}

Next, we present examples of DIBVs found by our analysis for each risky
operation category to provide a clear understanding of the traits of the
attacks. 

\paragraph{Risky memory access}

\begin{listing}[ht]
\begin{minted}[xleftmargin=21px, breaklines, linenos,fontsize=\small]{c}
static int ixgbe_ndo_fdb_add(..., const unsigned char *addr, ...)
{
    ...
    return ndo_dflt_fdb_add(ndm, tb, dev, addr, vid, flags);
}

int ndo_dflt_fdb_add(..., const unsigned char *addr, ...)
{
    int err = -EINVAL;
        ...
    else if (is_multicast_ether_addr(addr))
        err = dev_mc_add_excl(dev, addr);
        ...
    return err;
}

static inline bool is_multicast_ether_addr(const u8 *addr)
{
    ...
    u32 a = *(const u32 *)addr;
    ...
}
\end{minted}
\caption{Risky pointer dereference in ixgbe.}
\label{lst:risky_pointer_deref}
\end{listing}

In Linux's ixgbe driver, a potential risky memory access is in the
\texttt{ixgbe\_ndo\_fdb\_add} function
(Listing~\ref{lst:risky_pointer_deref}). This driver function can be
invoked by isolated code and passes an address to the kernel's
\texttt{ndo\_dflt\_fdb\_add} at line 4. The address is then dereferenced in
the \texttt{is\_multicast\_ether\_addr} function at line 11, triggering a
risky memory access at line 20. A driver can supply an invalid address,
allowing unauthorized memory reads or crashing the kernel.

\gtan{In this example, is it important to show
  \texttt{ixgbe\_ndo\_fdb\_add}, which is a driver function?  My
  understanding is that addr is shared data; so a malicious driver can
  just modify it arbitrarily. The same comment applies to later examples in this section.  }

\paragraph{Data used in risky API calls}
Our analysis of the ixgbe driver reveals several instances where data is
passed from the driver to the kernel, and subsequently used in potentially
risky API calls. An example of this is illustrated in
Listing~\ref{lst:ixgbe_risky_api_example}.

\begin{listing}[ht]
\fontsize{6}{11}\selectfont
\begin{minted}[xleftmargin= 21px,fontsize=\small,linenos,breaklines]{c}
void ixgbe_ptp_rx_pktstamp(struct ixgbe_q_vector q_vector, struct sk_buff skb)
{
    / ... /
    skb_copy_bits(skb, skb->len - IXGBE_TS_HDR_LEN, &regval, IXGBE_TS_HDR_LEN);
    / ... */
}

int skb_copy_bits(const struct sk_buff *skb, int offset, void to, int len) {
    / ... /
    skb_copy_from_linear_data_offset(skb, offset, to, copy);
    / ... */
}

static inline void skb_copy_from_linear_data_offset(const struct sk_buff *skb, const int offset, void *to, const unsigned int len)
{
    memcpy(to, skb->data + offset, len);
}
\end{minted}
\caption{ixgbe driver code invoking risky kernel API calls.}
\label{lst:ixgbe_risky_api_example}
\end{listing}

The driver function \texttt{ixgbe\_ptp\_rx\_pktstamp} (line 1) can be
invoked by the isolated driver code. This function subsequently invokes the
kernel function \texttt{skb\_copy\_bits} (line 7), passing the
\texttt{offset} and \texttt{to} pointer arguments. The key risky operation
is the \texttt{memcpy} call in
\texttt{skb\_copy\_from\_linear\_data\_offset} (line 17), which can be
triggered by the isolated driver calling \texttt{skb\_copy\_bits}. A
malicious driver could potentially supply an out-of-bounds \texttt{offset},
enabling it to read sensitive data beyond the packet buffer and leak it via
the \texttt{to} pointer. To prevent such attacks on kernel memory safety,
the isolation interface must properly validate shared state variables such
as \texttt{offset}.

\paragraph{Risky array index}
In Listing~\ref{lst:f_uac2_risky_array_access_example}, the risky operation
is an array access in \texttt{constrs\_interval} at line 23, which uses the
\texttt{var} parameter supplied by the \texttt{uac2\_pcm\_open} function in
the f\_uac2 usb audio  driver. \texttt{uac2\_pcm\_open} calls
\texttt{snd\_pcm\_hw\_constraint\_integer} and passes the \texttt{var}
parameter, which indexes into the \texttt{intervals} array in
\texttt{constrs\_interval}. A malicious driver could manipulate
\texttt{var} to cause an out-of-bounds access.

\begin{listing}[ht]
\begin{minted}[xleftmargin=21px, fontsize=\small,linenos,breaklines]{c}
// Isolated driver
int uac2_pcm_open() {
    // Initialize runtime
    struct snd_pcm_runtime *runtime;
    
    // Pass input to kernel
    snd_pcm_hw_constraint_integer(runtime, var);
}

// Kernel API
int snd_pcm_hw_constraint_integer(runtime, var) {
    // Get constraints
    struct snd_pcm_hw_constraints *constrs = &runtime->hw_constraints;
    // Var indexes array
    constrs_interval(constrs, var)
}

// Risky array indexing
struct snd_interval constrs_interval(constrs, var) {
    return &constrs->intervals[var - SNDRV_PCM_HW_PARAM_FIRST_INTERVAL];
}
\end{minted}
\caption{f\_uac2 driver supply risky array index value.}
\label{lst:f_uac2_risky_array_access_example}
\end{listing}



\paragraph{Risky branch condition}
\begin{listing}[ht]
\begin{minted}[xleftmargin=21px, fontsize=\small,linenos,breaklines]{c}
static int add_mc_to_global_list(struct mem_ctl_info *mci)
{
    struct list_head *item, *insert_before;
    struct mem_ctl_info *p;
    
    list_for_each(item, &mc_devices) {
        p = list_entry(item, struct mem_ctl_info, link);
        if (p->mc_idx >= mci->mc_idx) {
            if (unlikely(p->mc_idx == mci->mc_idx))
                goto fail1;
                ... 
        }
    }
fail1:
    ...
    return 1;
}


\end{minted}
\caption{Risky field used in branch.}
\label{lst:risky_branch_example}
\end{listing}

In the Linux kernel, the function add\_mc\_to\_global\_list is responsible
for adding a memory controller (mci) to a global list (mc\_devices) in a
sorted order based on the mc\_idx field. This mc\_idx field serves as an
identifier for the memory controller. However, if a malicious driver can
control the mc\_idx value of a mem\_ctl\_info structure, it can lead to
several potential issues.

Firstly, a Denial of Service (DoS) attack can be launched. If the malicious
driver sets mc\_idx to a value that already exists in the list, the
function will return early without adding the new mci to the list. This can
prevent legitimate memory controllers from being added to the list, leading
to a denial of service. Secondly, a resource exhaustion attack can occur.
If the malicious driver can repeatedly invoke this function with different
mc\_idx values, it could potentially exhaust system resources by filling up
the mc\_devices list. This could lead to system instability or even crashes
due to lack of resources.

\paragraph{Risky arithmetic operations}

\begin{listing}[ht]
\begin{minted}[xleftmargin=21px, fontsize=\small,linenos,breaklines]{c}
// driver function
static int net2272_plat_probe(struct platform_device *pdev)
{
    ...
    // resource_size_t is same as u64 type
    resource_size_t base, len;
    struct resource *iomem;
    ... 
    base = iomem->start;
    dev->base_addr = ioremap_nocache(base, len);
    ...
}

// kernel API
void __iomem *ioremap_nocache(resource_size_t phys_addr, unsigned long size)
{
    ...
    return __ioremap_caller(phys_addr, ...);
}

static void __iomem *__ioremap_caller(resource_size_t phys_addr, ...)
{
    ...
    last_addr = phys_addr + size - 1;
    if (!size || last_addr < phys_addr)
        return NULL;
    ...
}
\end{minted}
\caption{net2272 block driver supplies a base value to cause integer overflow on the last\_addr value used in a branch.}
\label{lst:net2272_risky_arith_op_example}
\end{listing}

Listing~\ref{lst:net2272_risky_arith_op_example} shows a potential integer
overflow in the kernel's memory mapping API \texttt{ioremap\_nocache},
which can be triggered by a driver. The driver function
\texttt{net2272\_plat\_probe} obtains a physical address \texttt{base} and
size \texttt{len} to map. It passes these values to
\texttt{ioremap\_nocache}. Inside \texttt{ioremap\_nocache}, the
\texttt{phys\_addr} and \texttt{size} are used to calculate
\texttt{last\_addr}, performing the addition \texttt{last\_addr =
phys\_addr + size - 1} at line 24. 

The check \texttt{if (!size || last\_addr < phys\_addr)} tries to detect
overflow by validating \texttt{last\_addr} is not less than the original
\texttt{phys\_addr}. If so, it returns \texttt{NULL}, potentially causing a
denial-of-service if unhandled. The key issue is the \texttt{phys\_addr}
and \texttt{size} values come directly from the isolated driver
compartment. A malicious or defective driver could provide crafted values
to trigger the integer overflow, and cause the remapping operation to fail. 
\fi

==> tex/defenses.tex <==

\iffalse
\section{Defenses}
In this section, we discuss some defenses that can be used on top of driver isolation to prevent certain types of DIBVs. 
TODO:
\begin{itemize}
\item Reading and writing from a wrong physical bus. e.g., pci, spi, i2c buses etc. 
\url{https://elixir.bootlin.com/linux/latest/source/drivers/pci/access.c#L413}
\item Do we correctly detect the aliases in these functions?
  \url{https://elixir.bootlin.com/linux/latest/source/drivers/net/ethernet/intel/ixgbe/ixgbe_main.c#L184}
  Specifically, we should establish that
  \lstinline{pdev->bus->parent->self} is aliased to the kernel
  parameter originally passed into \lstinline{probe} function
  \url{https://elixir.bootlin.com/linux/latest/source/drivers/net/ethernet/intel/ixgbe/ixgbe_main.c#L10826}
\end{itemize}
\fi

==> tex/design.tex <==
\subsection{Practices Beyond Driver Isolation}
\label{subsec:good_practice_for_enhancing_driver_isolation_security_guarantees}
Based on the analysis and the case study, we propose a set of good practices that driver isolation frameworks need to consider. These practices are derived from analyzing the \vulName{} at the kernel-driver isolation boundary. 

\paragraph{Practice 1: Minimize data sharing.} Defending the broad attack classes against the isolation boundary could be challenging, as it may require complicated policy enforcement. Yet, as we have shown, narrow down the shared data allows easier  on deriving policies and achieve better policy enforcement coverage, is to design the interface to minimize data sharing. While several existing driver designs generally follow this practice, e.g., by allocating private memory for driver data, we still have drivers that share excessive amount of data with kernel like ixgbe and nvme-core. This leads to our suggestion for the second practice below.

\paragraph{Practice 2: Develop tools to infer policies.} Given the challenging of deriving policies to enforce, developers can try to utilize or develop tools that can automatically infer policies. Such as using static analysis \cite{ksplit} to derive data accessing policies. This would make the policies more complete, and thus better realize the security guarantees the isolation frameworks provide.  

\paragraph{Practice 3: Address data invariants.} As we have seen, data-only attacks are still possible even when all the policies are correctly derived and enforced, as a data object which allows shared access may still violate invariants it should obey. This indicates that the current enforcement is not sufficient. In such cases, we have to derive the correct invariants, and make sure such invariants are enforced correctly. Computing all the correct invariants is generally an unsolvable problem, yet some tools such as Daikon can be used to infer the invariants, as demonstrated by previous work on inferring invariants at cross-domain boundary data\cite{protecting_comm_kernel_from_vulnerable_driver}.

\paragraph{Practice 4: Reusing invariants in the same driver class.} For drivers in the same class, they normally operate on the same shared data structures, e.g., struct net\_device in network drivers. Thus, the invariants that hold for one driver are likely to be transferable to other drivers in the same class. So, we should accumulate the invariants learned from protecting one driver, and reuse them for drivers in the same class. A good practice would be to formally document such invariants as part of general design guidelines for future driver development.  

\section{Evaluation Driver Isolation Defenses Against Attack Vectors}
In this section, we comprehensively discuss the defense mechanisms offered by existing driver isolation frameworks, and evaluate what attacks can be prevented with which isolation techniques.

Broadly speaking, we consider the driver isolation frameworks in the following broad categories: (1). Completely isolate device drivers to a different address space, and explicitly synchronize necessary data across the isolation boundary. (2). SFI based techniques, which intercept memory accesses and check if the access is valid. The summary of frameworks and their corresponding techniques are described in Table~\ref{tab:driver-iso-defense}. In a nutshell, memory isolation is shared across all the driver isolation framewroks. And on top of it, some other techniques are proposed to address potential interface vulnerabilities. Nooks only establish memory isolation. Microdriver and KSplit use static analyses to compute certain data access policies, and only synchronize the data that is needed. KSplit also compute shared data, establishing a stricter access policy compared with Microdriver. All these three frameworks uses shadow objects, and maintain a global map for object lookup. Such mechanisms can effectively prevents attacks that try to directly corrupts 
a kernel pointer, as the attackers only have access to the pointer at the driver side. The result of corrupting the driver pointer is causing loopup failure. In addition, since all kernel invocation is through rpc calls, a malicious driver, even with arbitrary code excution capability, cannot invoke arbitrary kernel functions, as only kernel interface functions with rpc stubs can be invoked properly. For a similar reason, driver also cannot trick the kernel to invoke arbitrary function through driver supplied function pointers, because any driver functions call back must has a rpc stub, and such stub cannot be modified by the attacker. Access control prevents potential oversharing. LXFI uses SFI to ensure driver code cannot access kernel memory region. On top of it, it uses capability to ensure the driver has valid access right to shared objects, e.g., write and reference capabilities.

